YOGA: Deep Object Detection in the Wild with Lightweight Feature Learning and Multiscale Attention

We introduce YOGA, a deep learning based yet lightweight object detection model that can operate on low-end edge devices while still achieving competitive accuracy. The YOGA architecture consists of a two-phase feature learning pipeline with a cheap linear transformation, which learns feature maps using only half of the convolution filters required by conventional convolutional neural networks. In addition, it performs multi-scale feature fusion in its neck using an attention mechanism instead of the naive concatenation used by conventional detectors. YOGA is a flexible model that can be easily scaled up or down by several orders of magnitude to fit a broad range of hardware constraints. We evaluate YOGA on COCO-val and COCO-testdev datasets with other over 10 state-of-the-art object detectors. The results show that YOGA strikes the best trade-off between model size and accuracy (up to 22% increase of AP and 23-34% reduction of parameters and FLOPs), making it an ideal choice for deployment in the wild on low-end edge devices. This is further affirmed by our hardware implementation and evaluation on NVIDIA Jetson Nano.

==> plots/plot10.tex <==
\begin{figure*}[ht]
    \centering
    
     \begin{minipage}[t]{0.5\linewidth}
         \centering
         \includegraphics[width=\linewidth]{fig/plot3-8.pdf}
         \caption{Plot of a training history (AP on the right Y axis).\vspace{7mm}}
         \label{figure:training}
     \end{minipage}\hfill
     \begin{minipage}[t]{0.5\linewidth}
         \centering
         \input{elsarticle/plots/plot3}
         \caption{Comparing YOGA with state-of-the-art OD models.}
         \label{figure:teaser}
    \end{minipage}
   

% From the image (a) and (b), we see that our model correctly detected the occluded object compared to YOLOv5. and from the (c) and (d) our model detected three more correct objects compared to YOLOv5 model     
   \vspace{-2mm} 
\end{figure*}


==> plots/plot2.tex <==
\pgfdeclareplotmark{mystar}{
    \node[star,star point ratio=2.25,minimum size=10pt,
    inner sep=0pt,draw=red,solid,fill=red] {};
}

\pgfdeclareplotmark{nabla}{
    \node[nabla,star point ratio=2.25,minimum size=5pt,
    inner sep=0pt,draw=orange,solid,fill=orange] {};
}

\begin{figure}[htbp]

\begin{tikzpicture}[][x=0.5pt,y=5pt,yscale=-1,xscale=1]

\begin{axis}[
	xlabel= \text{Number of parameters in Millions},
	ylabel= \text{AP},
	width= \linewidth,height=6cm,
	ylabel near ticks,
	xmin=0, xmax=90,
%    legend style={at={(1.05,0.95)}location=south east}
    legend pos= south east,
%    legend pos=outer north east,
 % (so the legend looks a bit better)
%    legend cell align=left,
    ]
% Add values and attributes for the first plot

\addplot[color=red, mark=mystar, thick, mark size=3pt] plot coordinates {
    (1.89, 32.3)
	(7.6, 40.7)
	(16.3, 45.2)
	(33.6, 48.9)
% 47.9 to 48.9
};

\addplot[thick,color=green,mark=*,mark size =3pt] plot coordinates {
     (1.9,28.4)
     (7.2,37.2)
     (21.2,45.2)
     (46.5, 48.8)
     };
     
%\addplot[color=black!40!green, mark=diamond*,mark size =3pt, thick] plot coordinates {
%    (0.9, 25.3)
%	(5.06, 32.8)
%	(9, 39.6)
%	(25.3,46.4)
%	(54.2, 50.0)
%};
\addplot[mark=triangle*, color=cyan, mark size=3pt, thick] plot coordinates {
	(4.4, 26.2)
	(5.7, 31.5)
	(7.3, 35)
	(11, 38.8)};
% Add values and attributes for the second plot

\addplot[mark=oplus,mark size=3pt,draw=orange,thick] plot coordinates {
   (4.20,22.7)
   (45,45.1)
% directly from paper
};


%\addplot[mark=square*,mark size =2.5pt,draw=orange,solid,fill=orange,thick] plot coordinates { (6.06,21.7)
% yolov4-csp (custom run)
%(52.9,48.64)
%};
%Raja: why there is a large gap between points of PPYOLO and Efficient-Det. I am looking into computing the other parameter values

\addplot[only marks,
      mark=text,
      text mark=A,
      text mark as node,
      text mark style={%
        font=\small,
        circle,
        inner sep=.05em,
        fill=blue!10!white,
        draw=blue,thick,
        fill=none
      }] plot coordinates {
 (6.06,21.7)
};



\addplot[only marks,
      mark=text,
      text mark=B,
      text mark as node,
      text mark style={%
        font=\small,
        circle,
        inner sep=.05em,
        fill=blue!10!white,
        draw=blue,thick,fill=none
      }] plot coordinates {
 (36.1,26.8)
};

\addplot[only marks,
      mark=text,
      text mark=C,
      text mark as node,
      text mark style={%
        font=\small,
        circle,
        inner sep=.05em,
        fill=blue!10!white,
        draw=blue,thick, fill=none
      }] plot coordinates {
(19, 21.2)
};

%\addplot[mark=*] plot coordinates {
%   (65.25,33.0)
%};
% removing YOLOv3 since it is not appearing as a good comparison in the plot (x axis is very high and y is very low)  

  
%\node [above] at (axis cs:  6,  22) {YOLOv4-Tiny};
\legend{YOGA, YOLOv5,EfficientDet-lite, PPYOLO,YOLOv4, SSD512, Faster-RCNN}
\end{axis}

\end{tikzpicture}

%\caption{Accuracy comparison of all state-of-the-art models  trained on the same resolution of $640 \times 640$ images.}
\caption{Comparing YOGA with state-of-the-art object detection models. %Each curve that consists of multiple data points represent different versions (tiny/nano, small, medium, and large) depending on the actual model size (X axis). %All the models are trained on the same image resolution of 640 $\times$ 640 (in fact the same dataset)
}
\label{fig:teaser}
\end{figure}

%\addplot[mark=square*,mark size %=2.5pt,draw=orange,solid,fill=orange,thick] plot coordinates {
%(41, 42.0)
%(60,44.9)
%};


==> tables/table6.tex <==
\begin{tabular}{ccc}
     \hline
{Backbone} & {Neck} &{AP} \\ \midrule
%     YOGA-\textit{n} & \checkmark & &  & 31.5\\
%     YOGA-\textit{n} & \checkmark & \checkmark & \checkmark & 32.1\\
     YOLOv5 Backbone & Naive Concat & 28.4 \\
     CSPGhostNet & Naive Concat & 31.1\\
     CSPGhostNet & AFF-PANet &  \textbf{32.3}\\
     \bottomrule
\end{tabular}


